PRAM: Place Recognition Anywhere Model for Efficient Visual Localization

Visual localization is a key technique to a variety of applications, e.g., autonomous driving, AR/VR, and robotics. For these real applications, both efficiency and accuracy are important especially on edge devices with limited computing resources. However, previous frameworks, e.g., absolute pose regression (APR), scene coordinate regression (SCR), and the hierarchical method (HM), have limited either accuracy or efficiency in both indoor and outdoor environments. In this paper, we propose the place recognition anywhere model (PRAM), a new framework, to perform visual localization efficiently and accurately by recognizing 3D landmarks. Specifically, PRAM first generates landmarks directly in 3D space in a self-supervised manner. Without relying on commonly used classic semantic labels, these 3D landmarks can be defined in any place in indoor and outdoor scenes with higher generalization ability. Representing the map with 3D landmarks, PRAM discards global descriptors, repetitive local descriptors, and redundant 3D points, increasing the memory efficiency significantly. Then, sparse keypoints, rather than dense pixels, are utilized as the input tokens to a transformer-based recognition module for landmark recognition, which enables PRAM to recognize hundreds of landmarks with high time and memory efficiency. At test time, sparse keypoints and predicted landmark labels are utilized for outlier removal and landmark-wise 2D-3D matching as opposed to exhaustive 2D-2D matching, which further increases the time efficiency. A comprehensive evaluation of APRs, SCRs, HMs, and PRAM on both indoor and outdoor datasets demonstrates that PRAM outperforms ARPs and SCRs in large-scale scenes with a large margin and gives competitive accuracy to HMs but reduces over 90\% memory cost and runs 2.4 times faster, leading to a better balance between efficiency and accuracy.

==> sections/introduction_v1.tex <==
\section{Introduction}
\label{sec:intro}



\input{tables/table_methods}

\begin{figure}[t]
	\centering
	%\includegraphics[width=.98\linewidth]{images/overview2}
	\includegraphics[width=1.\linewidth]{images/human_recognition}
	\caption{\textbf{Humans' efficient localization system}. Humans encode places as landmarks in the memory in a self-supervised manner. These places could be famous buildings such as Eiffel Tower and Kings College or common objects such as ovens. As these landmarks are associated with unique locations, when seeing them, humans know where they are.}
	\label{fig:human_recognition}
\end{figure}

\begin{figure*}[t]
	\centering
	%\includegraphics[width=.98\linewidth]{images/overview2}
	\includegraphics[width=1.\linewidth]{images/overview3}
	\caption{\textbf{Overview of our framework}. The reconstruction module recovers the 3D map from reference images and defines 3D landmarks hierarchically; the recognition module extracts sparse keypoints from the query image and predicts corresponding landmark labels with visual transformers; with recognized landmarks, the registration module performs landmark-wise 2D-3D matching to estimate the absolute pose of the query image (better view in color).}
	\label{fig:overview}
\end{figure*}

\IEEEPARstart{V}isual localization aims to estimate the rotation and position of a given image captured in a known environment. As a fundamental computer vision task, visual localization is the key technique to various applications such as virtual/augmented reality (VR/AR), robotics, and autonomous driving. After several decades of exploration, many excellent methods have been proposed and can be roughly categorized as absolute pose regression (APR)~\cite{posenet,posenet-geo2017,lsg,glnet,atloc2020,mapnet,sc-wls2022}, scene coordinate regression (SCR)~\cite{scr2013,dsac,ace2023,hscnet2020,dsac*}, and hierarchical methods (HM)~\cite{as,hfnet,lbr,as}. APRs implicitly embed the map into high-level features and predict the 6DoF pose with multi-layer perceptions (MLPs); they are fast especially for large-scale scenes, but have limited accuracy due to implicit 3D information representation. Unlike APRs, SCRs regress 3D coordinates for all pixels directly and estimate the pose with PnP~\cite{epnp} and RANSAC~\cite{ransac1981}. Despite the high accuracy in indoor environments, SCRs are hard to scale up to outdoor large-scale scenes. Instead of predicting 3D coordinates directly, HMs adopt global features~\cite{netvlad,patchnetvlad2021,gem2018} to search reference images in the database and then build correspondences between keypoints extracted from query and reference images. These 2D-2D matches are lifted to 2D-3D matches and used for absolute pose estimation with PnP~\cite{epnp} and RANSAC~\cite{ransac1981} as SCRs. Regardless of the outstanding accuracy and adaptability in large-scale scenes, HMs have high storage cost for global and local 2D descriptors of reference images and high time cost of global reference search and exhaustive 2D-2D matching especially when graph-based matchers~\cite{superglue,imp2023,sgmnet,clustergnn} are employed. In Table~\ref{tab:methods}, we list advantages and disadvantages of APRs, SCRs and HMs and want to ask:

\textit{Can we find an efficient and accurate solution to visual large-scale localization?}



We take the inspiration from humans' localization system. Humans localize themselves quickly by recognizing certain objects and their spatial relationships, as shown in Fig.~\ref{fig:human_recognition}. For example, The Eiffel Tower tells that we are in Pairs; the Kings College reveals that we are at the center of Cambridge city in UK; the oven implies we are in the kitchen. When uncertain about the recognition results, we align detailed structures of objects with those in our memory for verification. These techniques, if used for visual localization task, could significantly improve the efficiency especially in large-scale environments. However, it is not easy to achieve this because of two major challenges. The first one is how to define landmarks in the real world. Some previous works explore this by defining landmarks on object instances, e.g., building facades~\cite{lbr,localinstance}. Despite their promising performance in certain scenes, these methods can not be extended to any places like humans' recognition system. Instead, we seek from the 3D map which contains all places in the environment and adopt a hierarchical clustering strategy to define landmarks on 3D points directly. This allows us to make any place a landmark automatically without any laborious labeling and thus solve the first challenge. 

The second challenge is how to recognize a large number of landmarks efficiently. For example, the prediction layer outputs features with 512 Megabytes to recognize 512 landmarks for an image with size of $512\times512$, impairing the efficiency especially on edge devices with limited computational resources. To solve this problem, we propose to recognize landmarks of sparse keypoints as opposed dense pixels. Sparse keypoints~\cite{superpoint,sfd22023,sift,orb,r2d2,lift} such as corners and their spatial relationships effectively reveal the structure of objects~\cite{sparc2022,sparse2023} and hence can be used to replace dense but redundant pixels for recognition. Moreover, these keypoints are sparse tokens naturally, enabling us to leverage the more powerful transformers~\cite{attention2017} for recognition. 

In this paper, we propose the place recognition anywhere model (PRAM) for visual localization, as shown in Fig.~\ref{fig:overview}. We first use the local feature method SFD2~\cite{sfd22023} to extract sparse keypoints for 3D reconstruction; then we perform hierarchical clustering on reconstructed 3D points to define landmarks automatically in a self-supervised manner; finally, sparse keypoints along with their spatial relationships are used as tokens to be fed into a transformer-based recognition module to recognize landmark labels. At test time, sparse keypoints and their predicted landmarks are further used for fast semantic-aware registration between 2D keypoints and 3D points in the map for pose estimation. 

Compared with prior frameworks~\cite{posenet,glnet,dsac,hfnet}, PRAM has many advantages. (1) By recognizing landmarks, PRAM determines the coarse location with constant time and memory complexity as opposed to reference search with global descriptors, improving both the time and memory efficiency. (2) With predicted landmark labels, PRAM filters potential outlier keypoints which don't have corresponding 3D points in the map to avoid redundant computation. Note that if a 2D keypoint is an inlier or outlier is and only is determined by if it has corresponding 3D point in the map. Manual definitions from previous works~\cite{smc,lbr} such as, keypoints from buildings are inliers, those from trees not, don't generalize well. (3) Predicted landmarks allow the registration module to perform fast semantic-aware 2D-3D registration instead of lifting 2D-2D matches to 2D-3D matches in HMs~\cite{hfnet,lbr}. This further improves the time efficiency because a large amount of redundant 2D descriptors associated with reference images are discarded. (4) PRAM is flexible to be extended to multi-modality localization. Recognition makes localization a high-level perception task rather than a classic low-level task; any other signals such as GPS, texts, voices can be encoded as additional tokens to join keypoints for recognition enhancement. (5) Other inspirations from PRAM such as large-scale scene coordinate regression, robust keypoints selection for localization and map sparsification and so on will be discussed in Sec.~\ref{sec:open_problems} as open problems.

%image-based and structure-based approaches. Image-based systems estimate the pose of a query image by finding the most similar reference one in the database with global features~\cite{netvlad,gem2018} or predict the pose directly with a single network as Posenet~\cite{posenet} and its variants~\cite{lsg,glnet,mapnet}.

%initially, reconstruction of the map, a large database with global features and local features, known as structure-based approach. Due to its robust to appearance changes and accuracy in large-scale scenes, structure-based methods are widely used especially in industry. 

%With the development of deep learning, methods based on absolute pose regression (APR) and scene-coordinate regression (SCR) are proposed to reduce the memory and time cost. APR models~\cite{posenet} produce the pose with a single network in an end-to-end fashion. As no explicit 3D maps used for pose estimation, APRs perform like image retrieval task~\cite{sattler2019understanding} despite further improvements obtained from sequential enhancement~\cite{mapnet,lsg,glnet}, attentions~\cite{atloc2020}, rendering more training data~\cite{lens2022}, additional matching~\cite{dfnet2022}.

%SCR systems~\cite{dsac,dsac++,sc-wls2022} first predict the 3D coordinate of each pixel and then estimate the pose with the PnP~\cite{epnp} + RANSAC~\cite{ransac1981}.

%In spite of the improvements the aforementioned methods, challenges still exist. We demonstrate the strengths and weaknesses of these methods in Table.~\ref{}.  Table.~\ref{} demonstrates that classic structure-based methods have high accuracy and work well in large-scale scenes, but have high memory cost and slow. APRs are both time and memory efficient, but have limited accuracy~\cite{sattler2019understanding}. SCRs are memory efficient as well. However, they can hardly report competitive results in large-scale scenes. In this paper, we want to ask is it possible to design a new framework which are as accurate as structure-based methods and as efficient as APRs and SCRs in large-scale scenes?




%We are trying to achieve the this goal from the following aspects.

%\textbf{Map-centric localization.} One of the major differences between SbMs and APRs/SCRs is the former put images at the center and the latter put map at the center. SbMs rely on the images to provide global features~\cite{netvlad,patchnetvlad2021} or BoWs to find reference images, and local features~\cite{sift,superpoint,r2d2,sfd22023} to building 2D-2D correspondences. 2D-2D correspondences are then converted to 2D-3D matches between keyponints from the query image and 3D points observed by the reference image. By leveraging images and 2D keypoints as the bridge, SbMs avoid the challenging direct 2D-3D matching, but suffer from the huge memory cost of string global and local features and the additional time cost of searching reference images and 2D-2D matching. On the contrary, the SCRs embed the map into the network implicitly and report corresponding 3D coordinate for each pixel directly, reducing the memory and time cost significantly. While the precision of regression is limited in large-scale scenes.

%\textbf{Perception matters.} The ideal framework for visual localization is predicting the pose from a query image as Posenet~\cite{posenet}. However, due to missing of explicit correspondences, Posenet and its variants fail to give precise poses. SCRs step back to build correspondences with pixels and 3D coordinates and achieve much better accuracy. 

%\textbf{Geometric computation.} Although pose regression~\cite{posenet,lsg,glnet,deepfuntal2018} has achieved great progress, its accuracy is still limited compared to estimators with explicit correspondences. This is also the difference between ARPs and SCRs and the inferior accuracy of APRs. We believe that in the future an accurate pose could be obtained by a network in an end-to-end fashion, while at the moment explicit correspondences are still necessary for precise pose estimation. Therefore, when designing the framework, the geometric computation is retrained.

%In this paper, based on our intuition, we design a new framework for visual localization. First of all, instead of 2D semantics classes, we adopt a map-centric strategy and define landmarks directly on 3D map. By recognizing which landmark each keypoint belongs to, our framework avoids global reference search. Additionally, landmark recognition allows the system to work in large-scale environments without worrying about the regression precision. Second, after recognizing the landmarks, we perform 2D-3D matching with the guidance of class labels, making matching more efficient than brute-force specially for graph-based matchers~\cite{superglue,sgmnet,imp2023}. Finally, the 2D-3D correspondences are fed into the geometric computation module which combines PnP and RANSAC for absolute 6-DoF pose estimation. In our new framework, the memory size is only 5\% of a typical SbMs such as SPP+SPG+NetVLAD~\cite{superpoint,superglue,netvlad}, but gives competitive pose accuracy on large-scale Aachen-Day-Night dataset~\cite{aachen}.

%Our new framework contains two major components: perception and geometric computation and is named as PGNet. Compared with SbMs, PGNet discards global features and 2D features and hence is much more memory-efficient. Besides, PGNet finds potential landmarks by recognition in constant time as opposed to global reference search adopted by SbMs which has linear complexity to the number of reference images in the database. Moreover, with the guidance of landmark labels, PGNet significantly reduces the time of matching. As PGNet conducts recognition on landmarks, it is more robust than SCRs in large-scale environments.

Our contributions are concluded as follows:

\begin{itemize}
	\item We propose a new localization framework, called PRAM,  which allows us to do localization anywhere efficiently.
	
	\item We comprehensively analyze the accuracy and efficiency of APRs, SCRs, HMs and PRAM. Results demonstrate that PRAM outperforms APRs and SCRs in terms of accuracy in large-scale scenes and gives higher time and memory efficiency than HMs.
	
	\item PRAM opens a new direction for efficient and accurate large-scale localization such as muti-modality localization, sparse scene coordinate regression, map sparsification and so on.
\end{itemize}

Our experiments on indoor 7Scenes~\cite{sevenscenes2013}, 12Scenes~\cite{twelvescenes2016} datasets and outdoor CambridgeLandmarks~\cite{posenet} and Aachen~\cite{aachen} datasets demonstrate that PRAM is $50\times$ smaller and $2.4\times$ faster than previous state-of-the-art HMs~\cite{hfnet,lbr}. The rest the paper is organized as follows. We discuss related works in Sec.~\ref{sec:related_works} and introduce PRAM in detail in Sec.~\ref{sec:method}. We evaluate our method in Sec.~\ref{sec:experiemnt_setup} and Sec.~\ref{sec:experiemnts}. We discuss potential insights of our framework for visual localization in Sec.~\ref{sec:open_problems} and conclude the paper in Sec.~\ref{sec:conclusion}.
Our experiments on indoor 7Scenes~\cite{sevenscenes2013}, 12Scenes~\cite{twelvescenes2016} datasets and outdoor CambridgeLandmarks~\cite{posenet} and Aachen~\cite{aachen} datasets demonstrate that PRAM is $50\times$ smaller and $2.4\times$ faster than previous state-of-the-art HMs~\cite{hfnet,lbr}. The rest the paper is organized as follows. We discuss related works in Sec.~\ref{sec:related_works} and introduce PRAM in detail in Sec.~\ref{sec:method}. We evaluate our method in Sec.~\ref{sec:experiemnt_setup} and Sec.~\ref{sec:experiemnts}. We discuss potential insights of our framework for visual localization in Sec.~\ref{sec:open_problems} and conclude the paper in Sec.~\ref{sec:conclusion}.
Our experiments on indoor 7Scenes~\cite{sevenscenes2013}, 12Scenes~\cite{twelvescenes2016} datasets and outdoor CambridgeLandmarks~\cite{posenet} and Aachen~\cite{aachen} datasets demonstrate that PRAM is $50\times$ smaller and $2.4\times$ faster than previous state-of-the-art HMs~\cite{hfnet,lbr}. The rest the paper is organized as follows. We discuss related works in Sec.~\ref{sec:related_works} and introduce PRAM in detail in Sec.~\ref{sec:method}. We evaluate our method in Sec.~\ref{sec:experiemnt_setup} and Sec.~\ref{sec:experiemnts}. We discuss potential insights of our framework for visual localization in Sec.~\ref{sec:open_problems} and conclude the paper in Sec.~\ref{sec:conclusion}.



==> sections/open_problems.tex <==
\section{Limitations and Open Problems}
\label{sec:open_problems}

\begin{figure}[t]
	\centering
	\includegraphics[width=1.\linewidth]{images/sam_openvoc}
	\caption{\textbf{Results of SAM~\cite{sam2023} and open-vocabulary recognition}. Results of SAM provide object masks which can be used as object-level constraints in the hierarchical clustering process. These objects can be further assigned with semantic labels by open-vocabulary classification models, so that we can build a hierarchical semantic map at the same time.}
	\label{fig:sam_openvoc}
\end{figure}


PRAM is a new framework for visual localization, so many limitations and open problems exist. In this section, we discuss these limitations and open problems and hope following researchers can make PRAM better.

\textbf{Landmark definition.} Our current strategy of generating landmarks considers mainly the spatial connections of points. The object-level consistency is ignored, leading to the split of objects. In the future, we can use SAM~\cite{sam2023} results to provide additional object-level connections for 3D points during the hierarchical clustering process, avoiding this problem. Moreover, object labels can also be assigned by open-vocabulary classification models as shown in Fig.~\ref{fig:sam_openvoc}. In this way, we are able to build a hierarchical map of self-defined and commonly used semantic labels.

In addition to landmark definition, how to decide the number of landmarks is also important. In our experiments, we manually set the number of landmarks for different datasets according to their spatial size, which may not be optimal. An adaptive solution to determining the number of landmarks for a scene is worth of further exploration in the future.

\textbf{Map sparsification.} How to reduce map size including the number of reference images and 3D points remains a challenge in hierarchical frameworks. Previous methods~\cite{scenesqueezer2022,kcover2010,qp2013} rely mainly on the co-visibility between different reference images. Since images only represent the scene on 2D space rather than the 3D space, resulting in the loss of absolute scale, prior methods usually suffer from over-reduction, impairing the localization accuracy. However, PRAM performs sparsification on the landmarks defined on 3D points with absolute scale of the scene directly, allowing all 3D points to be taken into consideration. Then, by assigning each landmark a virtual reference image, PRAM discards the reference images. Our strategy of conducting sparsification on 3D points first and then reference images may bring insights to map sparsification in HMs.

% This map-centric strategy make the map compact because the scale of a scene is define the 3D map itself rather than other information such as reference images. It is simple and works well for both indoor~\cite{sevenscenes2013,twelvescenes2016} and outdoor scenes~\cite{posenet,aachen}. However, some objects are split into several pieces due to the missing consistency of objects, impairing the recognition performance.


\textbf{Map-centric localization.} The map contains a lot of useful information but its importance is ignored by previous methods~\cite{hfnet,lbr,as,smc,fgsn} relying purely on reference images. For example, we define the landmarks directly on 3D map as opposed images. Compared to perform semantic segmentation on images, this strategy generalizes well in any scenes and avoids the problem of labeling and dealing with multi-view inconsistency. Besides, the map also tells us which keypoints are inliers and which are not, so that it is not necessary to find a manually-defined metric with low generalization ability for discrimination.

Moreover, PRAM provides a unified framework with only sparse keypoints for recognition and registration. It simplifies previous hierarchical localization framework which requires separate global and local features for coarse and fine localization, independently. Therefore, as opposed to optimizing global and local features separately, PRAM allows us to optimize only local keypoints. In the future, how to extract fewer but more effectively keypoints for localization can be directly optimized with priors of the useful map.

\begin{figure}[t]
	\centering
	\includegraphics[width=1.\linewidth]{images/multi_recognition}
	\caption{\textbf{Multi-modality localization}. Sparse keypoints extracted from images contain only visual information. In addition to visual information, other signals such as multi-view inputs, GPS, texts can also be used to improve the localization performance as long as they are useful for recognition. The transformer-based recognition module flexibly accepts multi-modality data as input once these signals are encoded as high-level features. }
	\label{fig:multi_recognition}
\end{figure}

\textbf{Multi-modality localization.} In PRAM framework, recognition is the key to efficient and accurate large-scale localization. As the recognition module takes sparse tokens as input, any other signals such as multi-view images, GPS, electromagnetic signals, texts, voices can be flexibly encoded as tokens to enhance the recognition performance, so as to improve the localization accuracy as shown in Fig.~\ref{fig:multi_recognition}.

Let us take GPS as an example. In HMs, the benefit of GPS is squeezing the search space for finding reference images faster and more accurately in outdoor environments. At the same time, HMs have to face problems of inaccurate GPS signals due to the block of high buildings and missing signals in indoor environments, resulting in limited gains of using GPS for anywhere visual localization. However, GPS signals either inaccurate or not, can be used as priors to improve the recognition implicitly. When the GPS is not available in indoor scenes, the GPS token can replaced with a vector of zero values. This can be achieved efficiently and implicitly by recognition module. Such analysis can also be applied to other signals. In a nutshell, for HMs, the gains of using multi-module signals are limited compared to cost, but for PRAM, the gains could be much higher than cost.


\textbf{Large-scale scene coordinate regression.} SCRs cannot report accurate poses in outdoor scenes because of the pixel-wise recognition nature. This problem can be partially solved by the combination with PRAM. Specifically, each landmark in the map built by PRAM is a sub-scene with small scale where SCRs are able to give good results. In the localization process, first, the recognition module gives landmark labels indicating which sub-scene each point belongs to. Then, instead of predicting coordinates in an absolute large scale, SCRs could predict the relative coordinates to small-scale sub-scenes. Finally, the absolute coordinates can be recovered by combining the relative coordinates and sub-scene locations as:

\begin{align}
	X^{r}_1,...,X^{r}_n = f_{SCR}(p_1,...,p_n), \\
	L_1,...,L_n = f_{ViT}(p_1,...,p_n), \\
	X^{a}_i =  X^{r}_i + \Delta X_{L_i}. 
\end{align}

$X^{r}_i$ and $X^{a}_i$ are predicted relative and absolute coordinates for 2D point $p_i$. $\Delta X_{L_i}$ is the relative coordinate of landmark $L_i$ in the map. $f_{SCR}$ is a network for relative coordinate regression. Budvytis et al.~\cite{localinstance} try to regress relative coordinates to global instances defined on building facades, but it cannot work in any places as PRAM does. We believe the combination of SCRs and PRAM is worth of exploration in the future.


  

==> tables/table_12scenes.tex <==
\setlength{\tabcolsep}{3.pt}

\begin{table*}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lccccccccccccc}
			\toprule
			Method & kitchen1 & living1 & bed & kitchen2 & living2 &luke & gates362 & gates381 & lounge & manolis & 5a & 5b & Average\\
			AS~\cite{as} & 100 & 100 & 100 & 99.1 & 100 & 100 & 100 & 100 & 99.7 & 100 & 98.8 & 99.5 & 99.8 \\
			HLoc~\cite{hfnet} & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 100 & 99.5 & 100\\ 
			%DSAC 
			DSAC*~\cite{dsac} & 100 & 99.8 & 100 & 100 & 100 & 100 & 100 & 99.5 & 100 & 98.6 & 99.4 & 100 & 99.8 \\ 
			%ACE~\cite{ace2023} & 
			SFD2+IMP~\cite{sfd22023,imp2023} &  100 & 100 & 100 & 99.6 & 100 & 99.8 & 100 & 100 & 99.7 & 100 & 96.4 & 100 \\
			SP+SG~\cite{superpoint,superglue} & 100 & 100 & 100 & 99.6 & 100 & 99.8 & 100 & 100 & 99.7 & 100 & 97.8 & 100 & \\  
			\midrule
			%Ours & 
			\bottomrule
		\end{tabular}
\caption{\textbf{Localization accuracy on the RobotCar-Seasons dataset.} The best results are highlighted.}
\label{exp:tab:12scenes}
\end{table*}

==> tables/table_7scenes.tex <==
\setlength{\tabcolsep}{1.pt}

\begin{table}
	%\footnotesize
	%\tiny
	\scriptsize
	\centering
		\begin{tabular}{lcccccccc}
			\toprule
			Method & Chess & Fire &  Heads & Office & Pumpkin & Red Kitchen & Stairs & Average\\
			AS~\cite{as} & 99.9 & 99.8 &  100 & 98.6 & 99.6 & 99.8 &91.9 & 98.5 \\ 
			HLoc~\cite{hfnet} & 100 9&  99.4 &  100 &  100 &  100 & 98.6 &72.0 &  95.7 \\
			DSAC & 99.9 & 98.9 &99.8 &98.1 &  99.0 &  97.0 &  92.0 &  97.8 \\
			DSAC* & 99.6 &  96.9 & 99.5&   95.3 & 90.9& 96.4 &88.4 &  95.3 \\
			%ACE~\cite{ace2023} & 
			SFD2+IMP~\cite{sfd22023,imp2023} & 100 & 100 & 99.9 & 99.6 & 100 & 97.9 & 72.7 & \\
			SP+SG~\cite{superpoint,superglue} & 100 & 100 & 100 & 99.5 & 100 & 97.7 & 67.8 & \\  
			\midrule
			%Ours & 
			\bottomrule
		\end{tabular}
\caption{\textbf{Localization accuracy on the RobotCar-Seasons dataset.} The best results are highlighted.}
\label{exp:tab:7scenes}
\end{table}

==> tables/table_ablation.tex <==
\setlength{\tabcolsep}{1.2pt}

\begin{table}[t]
	%\footnotesize
	%\tiny
	%\scriptsize
	\centering
	\caption{\textbf{Ablation study.} We test the influence of different feature+matcher combinations (F+M), tracking, refinement, sparsification, descriptor dimension, and the number of candidate landmarks to pose accuracy.}
		\begin{tabular}{lcccccc}
			\toprule
			F+M & Sparsification & Tracking & Refinement & \#D & \#Landmarks & Acc$\uparrow$  \\
			\midrule
			SFD2+IMP & \xmark & \cmark & \xmark & 128 & 20 & 94.5\% \\
			SFD2+IMP & \cmark & \cmark & \xmark & 128 & 20 &  94.3\%\\
			SFD2+IMP & \cmark & \cmark & \cmark & 128 & 20 & 96.8\% \\
                SP+SG & \cmark & \cmark & \cmark & 256 & 20 & 75.5\% \\
            
			\midrule
			SFD2+IMP & \cmark & \cmark & \cmark & 64 & 20 & 94.9\% \\
			SFD2+IMP & \cmark & \cmark & \cmark & 32 & 20 & 94.3\% \\
			SFD2+IMP & \cmark & \cmark & \cmark & 0 & 20 & 15.8\% \\
			\midrule
			SFD2+IMP & \cmark & \cmark & \cmark & 128 & 10 & 95.3\% \\
			SFD2+IMP & \cmark & \cmark & \cmark & 128 & 5 & 95.1\%  \\
			SFD2+IMP & \cmark & \cmark & \cmark & 128 & 1 & 91.7\% \\
			\bottomrule
			
		\end{tabular}
\label{tab:ablation}
\end{table}

==> tables/table_cambridgelandmarks.tex <==
\setlength{\tabcolsep}{5pt}

\begin{table*}[t]
	%\footnotesize
	%\tiny
	%\scriptsize
	\centering
	\caption{\textbf{Localization accuracy on the CambridgeLandmarks dataset~\cite{posenet}.} We report the median position (cm), orientation ($^\circ$) errors and localization success ratio of pose errors within ($25cm, 2^\circ$). NA indicates values unavailable.}
		\begin{tabular}{llccccc|c}
			\toprule
			Group & Method & Kings College &  Great Court & Old Hospital & Shop Facade & St Marys Church & Average\\
			& & \multicolumn{6}{c}{$t (cm)\downarrow/R (^\circ)\downarrow/Percent (25cm, 2^\circ$)$\uparrow$} \\
			\midrule
			
			\multirow{5}{*}{APRs} & MapNet~\cite{mapnet} & 107 / 1.9 / NA & 785 / 3.8 / NA & 149 / 4.2 / NA & 200 / 4.5 / NA & 194 / 3.9 / NA & 163 / 3.6 / NA \\
			& PAEs~\cite{pae2022} & 90 / 1.5 / NA & NA / NA / NA &  207 / 2.6 / NA & 99 / 3.9 / NA & 164 / 4.2 / NA &  140 / 3.1 / NA\\
			& LENS~\cite{lens2022} & 33 / 0.5 / NA & NA / NA / NA & 44 / 0.9 / NA & 27 / 1.6 / NA & 53 / 1.6 / NA & 39 / 1.2 / NA \\	
            &DFNet~\cite{dfnet2022} & 43 / 0.9 / NA & NA / NA / NA & 46 / 0.9 / NA & 16 / 0.6 / NA & 50 / 1.5 / NA & 39 / 1.0 / NA \\
			& Posenet~\cite{posenet} & 88 / 1.0 / 0 & 683 / 3.5 / 0 & 88 / 3.8 / 0 & 157 / 3.3 / 0 & 320 / 3.3 / 0 & 163 / 2.9 / 0 \\
			&MS-Transformer~\cite{mstrasformer2021} & 83 / 1.5 / 3.5  & NA / NA / NA &  181 / 2.4 / 2.2  & 86 / 3.1 / 4.9  & 162 / 4.0 / 0.4 & 128 / 2.8 / 2.8\\
			&GLNet~\cite{glnet} & 59 / 0.7 / 3.4 & NA / NA / NA & 50 / 2.9 / 3.6 & 190 / 3.3 / 7.9 & 188 / 2.8 / 0.6 & 122 / 2.4 / 3.9 \\
            & NeFeS~\cite{nefes2024} & 37 / 0.5 / 30.6 & NA / NA / NA &  52 / 0.9 / 18.1 & 15 / 0.5 / 70.9 & 37 / 1.1 / 33.6 & 35 / 0.8 / NA \\
						
			\midrule
			\multirow{3}{*}{SCRs}
			& NeRF-loc~\cite{nerfloc2023} & 7 / 0.2 / NA & 25 / 0.1 / NA &  18 / 0.4 / NA & 11 / 0.2 / NA &  4 / 0.2 / NA & 13 / 0.2 / NA \\
			& HSCNet~\cite{hscnet2020} & 18 / 0.3 / NA & 28 / 0.2 / NA & 19 / 0.3 / NA & 6 / 0.3 / NA & 9 / 0.3 / NA & 16 / 0.3 / NA \\
            & SRC~\cite{src2022} & 39 / 0.7 / NA & 81 / 0.5 / NA & 38 / 0.5 / NA & 19 / 1.0 / NA & 31 / 1.0 / NA & 42 / 0.7 / NA\\
            & DSM~\cite{dsm2021} & 19 / 0.4 / NA & 43 / 0.2 / NA & 23 / 0.4 / NA & 6 / 0.3 / NA & 11 / 0.3 / NA & 21 / 0.3 / NA\\
             & NeuMap~\cite{neumap2023} &  14 / 0.2 / NA & 6 / 0.1 / NA & 19 / 0.4 / NA & 6 / 0.3 / NA & 17 / 0.5 / NA & 12 / 0.3 / NA\\
			& SC-WLS~\cite{sc-wls2022} &  14 / 0.6 / 68.2 & 164 / 0.9 / 7.3 & 42 / 1.7 / 23.1 &  11 / 0.7 / 76.7 & 39 / 1.3 / 34.0 & 27 / 1.0 / 42.0\\
            
			& DSAC*~\cite{dsac*} & 13 / 0.4 / 72.3 & 40 / 0.2 / 22.2 & 20 / 0.3 / 57.1 & 6 / 0.3 / 91.3 & 13 / 0.4 / 81.5 & 18 / 0.3 / 64.9\\	
			
			& ACE~\cite{ace2023} & 28 / 0.4 / 44.6  &  42 / 0.2 / 28.7  & 31 / 0.6 / 40.7 & 5 / 0.3 / 98.1 & 19 / 0.6 / 61.3 & 25 / 0.42 / 54.7 \\
			
			\midrule
			\multirow{3}{*}{HMs} & AS~\cite{as} & 24 / 0.1 / NA & 13 / 0.2 / NA & 20 / 0.4 / NA & 4 / 0.2 / NA & 8 / 0.3 / NA & 14 / 0.2 / NA \\	
			& PixLoc~\cite{backtofeature} & 14 / 0.2 / NA &  30 / 0.1 / NA &  16 / 0.3 / NA &  5 / 0.2 / NA & 10 / 0.3 / NA & 15 / 0.2 / NA\\	
			& SANet~\cite{sanet2019} &  32 / 0.5 / NA &  328 / 2.0 / NA &  32 / 0.5 / NA &  10 / 0.5 / NA & 16 / 0.6 / NA & 84 / 0.8 / NA\\
             & CrossFire~\cite{crossfire} & 47 / 0.7 / NA & NA / NA / NA & 43 / 0.7 / NA & 20 / 1.2 / NA & 39 / 1.4 / NA & 37 / 0.7 / NA \\ 
			& DSM~\cite{dsm2021} & 19 / 0.4 / NA & 43 / 0.2 / NA & 23 / 0.4 / NA & 6 / 0.3 / NA & 11 / 0.3 / NA & 20 / 0.3 / NA \\
           
            & InLoc~\cite{inloc} & 46 / 0.8 / NA & 120 / 0.6 / NA & 48 / 1.0 / NA & 11 / 0.5 / NA & 18 / 0.6 / NA & 49 / 0.7 / NA \\
           
            & NeRFMatch~\cite{nerfmatch} & 13 / 0.2 / NA & 20 / 0.1 / NA & 21 / 0.4 / NA & 9 / 0.4 / NA & 11 / 0.4 / NA & 15 / 0.3 / NA \\
            & VRS-NeRF~\cite{vrsnerf2024} & 9 / 0.1 / 90.7  & NA / NA / NA & 11 / 0.2 / 79.7 &  2 / 0.1 / 96.1 & 5 / 0.2 / 90.8 & 7 / 0.2 / 89.3\\
			& SFD2+IMP~\cite{sfd22023,imp2023} & 7 / 0.1 / 94.8 & 11 / 0.1 / 74.6 & 10 / 0.2 / 80.2 & 2 / 0.1 / 97.1 & 4 / 0.1 / 98.7 & 7 / 0.1 / 89.1\\
			& SP+SG~\cite{superpoint,superglue} & 7 / 0.1 / 94.5 & 12 / 0.1 / 74.7 & 9 / 0.2 / 81.9 & 2 / 0.1 / 97.1 & 4 / 0.1 / 98.7 & 7 / 0.1 / 89.4\\  
			
			\midrule
			& \textbf{Ours} & 15 / 0.1 / 71.1 & 16 / 0.1 / 62.5 & 9 / 0.2 / 78.0 & 2 / 0.1 / 98.1 & 5 / 0.2 / 96.8 & 9 / 0.1 / 81.3\\
			\bottomrule
		\end{tabular}

\label{tab:cambridgelandmarks}
\end{table*}

==> tables/table_landmarks.tex <==
\setlength{\tabcolsep}{10.pt}

\begin{table}
	%\footnotesize
	%\tiny
	%\scriptsize
    \caption{\textbf{The number of landmarks in different datasets.} For 7Scenes and 12Scenes datasets, we assign each scene 16 landmarks and therefore obtain up to $112 = 7\times16$ and $192 = 12 \times 16$ landmarks, respectively. Each scene in CambridgeLandmarks dataset has 32 landmarks, so this dataset has $160 = 5 \times 32$ landmarks in total. Aachen has only one scene with 512 landmarks.}
	\centering
		\begin{tabular}{lcc}
			\toprule
			Dataset & \#Scenes & \#Landmarks \\
			\midrule
			7Scenes (S)~\cite{sevenscenes2013} & 7 & 112 \\
			12Scenes (T)~\cite{twelvescenes2016} & 12 & 192 \\
			CambridgeLandmarks (C)~\cite{posenet} & 5 & 160 \\
			Aachen (A)~\cite{aachen} & 1 & 512 \\
			%RobotCar (R)~\cite{robotcar} & 1 & 512 \\
			%\midrule
			%CAST~\cite{sevenscenes2013,twelvescenes2016, aachen, posenet} & 25 & 976\\
			\bottomrule
		\end{tabular}
\label{tab:landmarks}
\end{table}
